Profit Sharing Contracts between Content and Service Providers for Enhanced Network Quality

It has been a long demand of Internet Service Providers (ISPs) that the Content Providers (CPs) share their profits for investments in network infrastructure. In this paper, we study profit sharing contracts between a CP with multiple ISPs. Each ISP commits to improving the Quality of Service (QoS) for the end-users through higher investments efforts. The CP agrees to share the profits due to the resulting higher demand for its content. We first model non-cooperative interaction between the CP and the ISPs as a two-stage Stackelberg game. CP is the leader that decides what fraction of its profits will be shared with the ISPs. Each ISP then simultaneously decides the amount of effort (investment) to enhance network quality. Here, CP cannot observe individual effort by the ISPs, which poses a challenge for the CP to decide how to share the profits with each ISP. Therefore, we also investigate a cooperative scenario, where the CP only decides the total share it gives to the ISPs, and each ISP then cooperatively shares the profit among themselves. We study the effect of such cooperation between the ISPs by building a Nash Bargaining based model. We show that the collaboration improves total effort by the ISPs and the payoff of the CP.

==> Extra/NBP-sectionIII.tex <==
\subsection{Cooperation scenario}
In this section, we study the case of a cooperative scenario where given the constant effort by $ISP_1$, $ISP_2$ maximizes the joint utility of both ISPs to make the effort decision to improve the QoS for CP’s content. Further, CP pays a revenue share to ISPs jointly, and ISPs cooperatively decide the split between them. There are two stages under this case.
\begin{itemize}
    \item \textit{Stage 1:} CP first announces a total share $\beta$ for both ISPs and $ISP_2$  maximizes the sum utility of both ISPs taking into account the constant effort level $\overline{a}_1$ of $ISP_1$. 
    \item \textit{Stage 2:} ISPs cooperatively decide the split of revenue share $\beta$, that depends on both effort, between them. We consider the outcome of splitting the share proportion $\beta$ by using the well-known cooperative solution concept of the \textit{Nash Bargaining solution}  (NBS). Nash Bargaining problem helps two players decide how to share a surplus generated by their joint actions. This solution concept satisfies important axioms which are: invariant to affine transformations, Pareto optimality, independence of irrelevant strategies and symmetry [8]. 
\end{itemize}

%In the following subsections, we consider our problem stage wise: Stage 1 followed by Stage 2.

%We consider two different cooperative settings- (i) Nash Bargaining and (ii) Shapley Value. We analyze the two settings as in bargaining, one players may contribute more to the coalition than other or may possess different bargaining power, while Shapley value gives final distribution of generated surplus among the players according to their contribution in the coalition. 
\subsubsection{Stage 1}
Stage 1 problem constitutes joint payment of revenue share by CP to ISPs, and joint utility maximization by $ISP_2$ to make effort decision (given fixed $\overline{a}_1$). The problem for Stage 1 is given as follows:\\
CP:\\
$$\max_{\beta\in[0,1]} \quad (1-\beta)r\log(\overline{a}_1+a_2+1)$$	
Since, $ISP_1$ puts constant effort $\overline{a}_1$, the joint maximization problem for $ISP_2$ is given by\\
$$\max_{a_2} \quad \beta r\log(\overline{a}_1+a_2+1)-c_1\overline{a}_1-c_2a_2$$
The best response $a_2(\beta)$ by $ISP_2$ in response to the contract offered by CP is given such that: 
\begin{equation}
a_2(\beta)= \frac{\beta r}{c_2}-1-\overline{a}_1.
	%	 \quad \text{or} \quad 	a_1+a_2=\frac{\beta r}{c_2}-1
\end{equation}
Following Theorem gives equilibrium revenue share proportion by CP.
\begin{thm} \label{thm:beta-2}
	The equilibrium contract between CP and ISPs given by 
	\begin{equation} \label{beta-nbs1}
		\beta= \frac{1}{W\left(\frac{r e }{ c_2}\right)}
	\end{equation}	
	%	\beta=\begin{cases} \frac{1}{W\left(\frac{r e }{ c_1}\right)} &\mbox{ if } \log\left(\frac{c_2}{c_1}\right)\ge \frac{c_1-c_2}{c_1}, \\ \frac{1}{W\left(\frac{r e }{ c_2}\right)} &\mbox{otherwise} \end{cases} 
\end{thm}
\textcolor{red}{This $\beta$ is same as $\beta_2$ in competitive scenario, which means CPs share less with ISPs now.}\\

Given, equilibrium share proportion from Theorem \ref{thm:beta-2}, one can now characterize the equilibrium effort by $ISP_2$ by the following corollary.
\begin{cor}
	The effort by $ISP_2$ at equilibrium is given by
	\begin{equation}
		a_2=\frac{r}{c_2W\left(\frac{r e }{ c_2}\right)}-\overline{a}_1-1
	\end{equation}
	\end{cor}
	\textcolor{red}{Here, the total effort is same as in competitive scenario. The total effort being same while less $\beta$ doesn't make sense for ISPs to cooperate as they will always get less payoff.}
\subsubsection{Stage 2}
Under this stage, ISPs can interact
and bargain with one another to arrive at a vector of revenue sharing contracts offered by CP, $(\beta_1^B,\beta_2^B)$, known as Nash Bargaining solution (NBS). Formally, the NBS $(\beta_1^B, \beta_2^B)$ is
defined as the solution of the following optimization problem:
$$\max_{\beta_1,\beta_2\in[0,1]} \quad \left(U_{ISP_1}(\beta_1)-d_{ISP_1}\right)\left(U_{ISP_2}(\beta_2)-d_{ISP_1}\right)$$
subjected to
$$U_{ISP_1}(\beta_1)\ge d_{ISP_1},$$
$$U_{ISP_2}(\beta_2)\ge d_{ISP_2}.$$

%\textcolor{}{where $U_{ISP_i}(\beta_i)=\beta_i\log(\overline{a}_1+a_2+1)-c_ia_i$ is the utility of $ISP_i$.

\textcolor{red}{how to define disagreement point now? As if we define disagreement to be competitive scenario, there will be no solution to NBP.}\\

The disagreement point $(d_{ISP_1},d_{ISP_2})$ is taken to the utilities
corresponding to the case of competitive scenario given by Corollary 1.

The NBS gives the split of $\beta$ given in eqn. (\ref{beta-nbs1}) between ISPs. Specifically, the NBS ($\beta_1^B, \beta_2^B$) can be written as $\beta_1^B,\beta-\beta_2^B$ since $\beta=\beta_1^B+\beta_2^B$. Thus, the Nash Bargaining problem can be written as follows:
\begin{align}\nonumber
	\max_{\beta_1^B} \quad \{\beta_1^Br\log(\overline{a}_1+a_2+1)&-c_1\overline{a}_1-d_1\}\times\\ \nonumber
	\{(\beta-\beta_1^B)&r\log(\overline{a}_1+a_2+1)-c_2a_2-d_2\}\\ \nonumber
		\text{subjected to}\hspace{10mm}&\\ \nonumber
	\beta_1^Br\log(\overline{a}_1+a_2+1)&-c_1\overline{a}_1\ge d_1\\ \nonumber
	(\beta-\beta_1^B)r\log(\overline{a}_1+a_2+1)&-c_2a_2\ge d_2
\end{align}
where $d_i=d_{ISP_i}, i=1,2$








\begin{comment}
\textcolor{black}{\begin{thm} \label{thm:nbs-1}
The NBS for the division of revenue share proportion between ISPs is given by 
	\begin{equation}
		(\beta_1^B,\beta_2^B)=\left(\frac{\beta}{2}-\frac{c_2a_2-c_1\overline{a}_1+d_2}{2r\log\left(\frac{\beta r}{c_2}\right)}, \frac{\beta}{2}+\frac{c_2a_2-c_1\overline{a}_1+d_2}{2r\log\left(\frac{\beta r}{c_2}\right)} \right) 
	\end{equation}	
	or
		\begin{equation}
		(\beta_1^B,\beta_2^B)=\left(\frac{c_1\overline{a}_1}{r\log\left(\frac{\beta r}{c_2}\right)}, \frac{c_2a_2+d_2}{r\log\left(\frac{\beta r}{c_2}\right)} \right) 
	\end{equation}		
\end{thm}}	
\end{comment}
%\subsubsection{Shapley Value}
%To decide how $\beta$ should be shared between ISPs, in this section, we use a different concept from coalitional theory, the Shapley value formula \cite{???}.	Shapley Value is a concept for ”fair” profit-sharing in cooperative game theory and we apply in Stage 2 of our game. The Shapley Value payoff to each ISP is determined by the average increment in profit that is due to its inclusion in the coalition, with the average computed over all possible coalitions.  It is the unique distribution satisfying the following axioms: efficiency (i.e., the total surplus is allocated), symmetry (i.e., players having the same contribution in the coalition are paid equally), dummy (i.e., players that do not have a contribution in the considered coalition are not paid), and additivity (i.e., if a game is composed of two sub-games, players are paid the sum of their shares in both sub-games). Therefore, each player receives a profit share proportional to its contribution in the network setting and the added value it brings to the overall system.

%	In the following Theorem, we compute the Shapley value.
%\begin{thm} \label{thm:SV-1}
%	The Shapley Value for ISPs is given by
%	\begin{align*}
%		\Phi_{ISP_1}&=\frac{1}{2}\left[r\left(1-\frac{2}{W\left(\frac{re}{c_1}\right)}\right)+c_1+a_1^*(c_2-c_1)\right]
%	\end{align*}
%	\begin{align*}
%		\Phi_{ISP_2}&=\frac{1}{2}\left[r\left(1-\frac{4}{W\left(\frac{re}{c_2}\right)}+\frac{2}{W\left(\frac{re}{c_1}\right)}\right)+(a_1^*+1)(c_2-c_1)\right]
%	\end{align*}
%\end{thm}

==> Extra/alternate.tex <==
\textcolor{red}{Alternate way:}\\
Problem is given by \\
CP:\\
$$\max_{\beta_i\in[0,1]\sum_i\beta_i\le 1} \quad (1-\beta_1-\beta_2)r\log(a_1+a_2+1)$$	
$ISP_i$\\
$$\max_{a_i} \quad \beta_ir\log(a_1+a_2+1)-c_ia_i$$
The best response by $ISP$'s in response to the contract offered by CP is given by 
\begin{equation}
	a_1+a_2= \frac{\beta_1 r}{c_1}-1
\end{equation}
and
\begin{equation}
	a_1+a_2=\frac{\beta_2 r}{c_2}-1
\end{equation}
This implies
\begin{equation} \label{betaratio}
	\frac{\beta_1}{\beta_2}=\frac{c_1}{c_2}
\end{equation}
Given this, the optimal strategy for CP is to offer the contract that maximizes
its utility, i.e., the solution to
\begin{equation} 
	\max_{\beta_i\in [0,1], \sum_i\beta_i\le 1} (1-\beta_1-\beta_2)\log \left(\frac{\beta_1 r}{c_1}\right)
\end{equation}
Using eqn. (\ref{betaratio}), we get \begin{equation} \label{opti}
	\max_{\beta_i\in [0,1]} \left(1-\beta_1\left(\frac{c_1+c_2}{c_1}\right)\right)\log\left(\frac{\beta_1 r}{c_1}\right)
\end{equation}


\textbf{Theorem:} \textit{The equilibrium contract between CP and $ISP_i, i=1,2$; is given by
	$$\beta_i=\frac{c_i}{(c_1+c_2)W\left(\frac{r}{c_1+c_2}e\right)}$$}


Now, we assume that $ISP_1$	always plays a fixed strategy say $\overline{a}_1$, then equilibrium strategy by $ISP_2$ is given by

\begin{equation}
	a_2=\frac{r}{(c_1+c_2)W\left(\frac{r }{c_1+c_2}e\right)}-\overline{a}_1-1
\end{equation}

Here we get
$$U_{CP}=\frac{\left[W\left(\frac{r }{c_1+c_2}e\right)-1\right]^2}{W\left(\frac{r }{c_1+c_2}e\right)}r$$

Now, 
\begin{align*}
	U_{ISP_1}&=\beta_1r\log(\overline{a}_1+a_2+1)-c_1\overline{a}_1\\
	&=\frac{c_1r}{(c_1+c_2)}\left(1-\frac{1}{W\left(\frac{r }{c_1+c_2}e\right)}\right)-c_1\overline{a}_1
\end{align*}
and
\begin{align*}
		U_{ISP_2}&=	\beta_2r\log(\overline{a}_1+a_2+1)-c_2a_2\\
	&=\frac{c_2r}{(c_1+c_2)}\left(1-\frac{2}{W\left(\frac{r }{c_1+c_2}e\right)}\right)+c_2\overline{a}_1+c_2
\end{align*}

\begin{thm} \label{ISP1}
Playing a constant strategy can give better payoff for $ISP_1$ as compared to $ISP_2$ iff 
\begin{align*}
 \overline{a}_1\le a_1^T
\end{align*}
where
\begin{align*}
 a_1^T =&\frac{r}{c_1^2-c_2^2}\left[c_1\left(1-\frac{1}{W\left(\frac{r }{c_1+c_2}e\right)}\right)\right.\\
 &\left.-c_2\left(1\frac{2}{W\left(\frac{r }{c_1+c_2}e\right)}\right)\right]-\frac{c_2}{c_1-c_2}.
\end{align*}
\end{thm}
\normalsize
Theorem \ref{ISP1} implies by acting non-strategically, and setting $\overline{a}_1$ below the threshold $a_1^T$, $ISP_1$ can achieve higher utility than $ISP_2$. As $ISP_1$ always puts constant effort, irrespective of action by $ISP_2$, it can still benefit and attain higher utility than $ISP_2$. This means being non-strategic may benefit $ISP_1$. 

We now consider the special case, where $\overline{a}_1$ is a solution of a particular optimization problem.  In fact, we consider the Stackelberg equilibrium solution concept between CP and $ISP_1$. This Stackelberg game between CP and $ISP_1$ is described as follows:\\
CP (leader):
$$\max_{\beta} \quad (1-\beta)r\log(a_1+1)$$
$ISP_1$ (follower):
$$\max_{a_1} \quad \beta r\log(a_1+1)-c_1a_1$$

\begin{proposition}
The unique equilibrium solution of the Stackelberg game between CP and $ISP_1$ is given by:\\
......
\end{proposition}

Under this case, we have the following result. 
\begin{lma} \label{ase}
If $\overline{a}_1=a_1^{SE}$, where $a_1^{SE}=\frac{\frac{r}{c}}{W\left(\frac{r}{c}e\right)}-1$ is Stackelberg Equilibrium when the contract is only between CP and $ISP_1$, then optimal effort by $ISP_2$ is $a_2^*=0$.
\end{lma}
From the above Lemma, it can be seen that if $ISP_1$ puts effort which is same is the equilibrium of the Stackelberg game between the CP and $ISP_1$, then there is no incentive for $ISP_2$ to put effort and it will free ride on the contribution of $ISP_1$. This is because $a^{SE}_1$  is higher than the total effort in case of the contract between the CP and both ISPs.


==> Extra/multiCP.tex <==
In this section, we consider the case of when there are multiple CPs, denoted as $CP_j; j=1,2$ connecting to end-users through ISPs, denoted as $ISP_i; ;i=1,2$. Each CP offers contract to both ISPs that connect end-users to the content of the CP. $ISP_i$ chooses to make investment decision $a_i^j; i, j=1,2$ for $CP_j$ and $CP_j$ shares the proportion of its revenue $\beta_i^j$ with $ISP_i$.

The increment in the demand $D_j$ for the content of $CP_j$ depends on the efforts $a_i^j$'s made by each $ISP_i$ and is given by $D_j := \log(a_1^j+a_2^j+1)$. The resulting revenue (increment) for $CP_j$ due to effort by each $ISP_i$ is given by $X_j := r_jD_j$, where $r_j$ is a constant that captures how each additional unit of demand translates to earnings. Thus, the revenue generated by $CP_j$ is then $X_j= r \log(a_1^j+a_2^j+1)$. 

	Thus, the utility of CP in this model is given by:
	$$U_{CP_j}=(1-\beta_1^j-\beta_2^j)r\log(a_1^j+a_2^j+1)$$
	and the utility of $ISP_i$ is:
	$$U_{ISP_i}=\sum_{j=1}^2\left(\beta_i^jr_j\log(a_1^j+a_2^j+1)-c_ia_i^j\right)$$
We consider a leader-follower interaction, with the each CP acting as a leader and ISPs as followers. The CP lead by announcing the revenue sharing contract, i.e., $CP_j$ offers the contract $\beta_i^j; i=1,2, j=1,2$ to the $ISP_i$. Each $ISP_i$ then responds to these contracts by determining its effort $a_i^j; i =1,2$.Then, the problem is given as	follows:\\
$CP_j; j=1,2$ (leader):
$$\max_{\beta_i^j \in [0,1], \sum_j \beta_i^j \le 1} \quad (1-\beta_1^j-\beta_2^j)r\log(a_1^j+a_2^j+1) $$
$ISP_i; i=1,2$ (follower):
$$\max_{a_i^j} \quad \sum_{j=1}^2\left(\beta_i^jr_j\log(a_1^j+a_2^j+1)-c_ia_i^j\right)$$
\subsection{Competitive scenario}
In this section, we consider the competitive scenario where each $CP_j$ make individual payment to each $ISP_i$ and each player acts strategically. Thus, the optimal effort by ISPs in response to the contract offered by $CP_j; j=1,2$ is given by
	$$ a_1^j+a_2^j= \frac{\beta_1^j r_j}{c_1}-1\quad \forall j=1,2$$
	and
	$$ a_1^j+a_2^j=\frac{\beta_2^j r_j}{c_2}-1\quad \forall j=1,2$$
	which implies 
	$$  \frac{\beta_1^j}{\beta_2^j}=\frac{c_1}{c_2} \quad \forall j=1,2$$
	Given this, the optimal strategy for $CP_j$ is to offer the contract that maximizes its utility, i.e., the solution to
	$$
	\max_{\beta_i^j\in [0,1], \sum_i\beta_i^j\le 1} (1-\beta_1^j-\beta_2^j)\log \left(\frac{\beta_1^j r_j}{c_1}\right)
	$$
	
The following result characterizes the equilibrium contracts between the $CP_j; j=1,2$
	and each $ISP_i; i=1,2$. .
	\begin{thm} 
		The equilibrium contract between $CP_j$ and $ISP_i$ is given by
		$$\beta_i^j=\frac{c_i}{(c_1+c_2)W\left(\frac{r_j}{c_1+c_2}e\right)}; i=1,2, j=1,2 $$
	\end{thm}
	Using above Theorem, and regulatory intervention that $\frac{a_1^j}{a_2^J}=\frac{\beta_1^j}{\beta_2^j}$, one can characterize the equilibrium effort of ISPs.
	\begin{cor}
		The equilibrium effort by $ISP_i^j$ is given by:
		$$ a_i^j=\frac{c_i}{c_1+c_2}\left[\frac{r_j}{(c_1+c_2)W\left(\frac{r_j }{c_1+c_2}e\right)}-1\right] \quad \forall i,j=1,2$$
	\end{cor}
	\subsection{Cooperative scenario}
	In this section, we consider the cooperative scenario between ISPs.ISPs jointly determine the effort for CPs, each CP makes joint payment to ISPs and ISPs cooperatively decide the split of the revenue share between them cooperatively through Nash Bargaining. Likewise considered in earlier sections, here also we have two stages. 
	
	
	
	\subsubsection{Stage 1:} Here, the problem for is given as follows:
	$CP_j, j=1,2$:\\
$$\max_{\beta^j \in[0,1]} \quad (1-\beta^j)r\log(a_1+a_2+1)$$	
ISPs\\
$$\max_{a_1, a_2} \quad \beta^j r\log(a_1+a_2+1)-c_1a_1-c_2a_2$$
The best response by ISPs in response to the contract offered by $CP_j$ is given by 
\begin{equation}
	a_1^j+a_2^j= \frac{\beta^j r_j}{c_1}-1 \quad \text{or} \quad 	a_1^j+a_2^j= \frac{\beta^j r_j}{c_2}-1 
\end{equation}
\begin{thm}
	The equilibrium contract between $CP_j, j=1,2$ and ISPs given by 
	\begin{equation}
	\beta^j=\begin{cases} \frac{1}{W\left(\frac{r_j e }{ c_1}\right)} &\mbox{ if } 	a_1+a_2= \frac{\beta^j r_j}{c_1}-1, \\ \frac{1}{W\left(\frac{r_j e }{ c_2}\right)} &\mbox{ if } 	a_1+a_2= \frac{\beta^j r_j}{c_2}-1 \end{cases} 
	\end{equation}	
	\end{thm}
	Using constraint $\frac{a_1^j}{a_2^j}=\frac{\beta_1^j}{\beta_2^j}$, we obtain equilibrium efforts by ISP, given by following Corollary. 
\begin{cor}
	The effort by ISPs for $CP_j$ at equilibrium is given by
	\begin{align} \nonumber
	    a_i^j&=\frac{c_i}{c_1+c_2}\left[\frac{r_j}{c_1W\left(\frac{r_j }{c_1}e\right)}-1\right] \\ \nonumber
	    &\text{or}\\
	    a_i^j&=\frac{c_i}{c_1+c_2}\left[\frac{r}{c_2 W\left(\frac{r_j }{c_2}e\right)}-1\right] \nonumber
	\end{align}

\end{cor}

\subsubsection{Stage 2} Now, in stage 2, the Nash Bargaining solution gives the split of revenue share proportion received from each $CP_j; j=1,2$ for ISPs. The problem is given by:
\begin{align}\nonumber
	\max_{\beta_1^j} \quad \{\beta_1^jr\log(a_1^j+a_2^j+1)&-c_1a_1^j-d_1^j\}\times\\\nonumber
	\{(\beta-\beta_1^j)&r\log(a_1^j+a_2^j+1)-c_2a_2-d_2^j\}\\\nonumber
	\text{subjected to}\hspace{10mm}&\\ \nonumber
	\beta_1^jr\log(a_1^j+a_2^j+1)&-c_1a_1^j\ge d_1^j\\ \nonumber
	(\beta-\beta_1^j)r\log(a_1^j+a_2^j+1)&-c_2a_2^j\ge d_2^j
\end{align}
where $d_i^j$ is the utility of $ISP_i; i=1,2$ under competitive scenario due to revenue share received from $CP_j; j=1,2$. Solving the problem gives following result.
\textcolor{}{\begin{thm} The NBS for the split of revenue share proportion received from $CP_j$ between ISPs is given by \\
If $a_1^j+a_2^j= \frac{\beta^j r_j}{c_1}-1$
	\begin{equation}
		(\beta_1^{jB},\beta_2^{jB})=\left(\frac{\beta^j}{2}-\frac{c_2a_2^j-c_1a_1^j+d_2^j-d_1^j}{2r\log\left(\frac{\beta^j r_j}{c_1}\right)}, \frac{\beta}{2}+\frac{c_2a_2-c_1a_1+d_2^j-d_1^j}{2r\log\left(\frac{\beta^j r_j}{c_1}\right)} \right) 
	\end{equation}	
	or
	\begin{equation}
		(\beta_1^{jB},\beta_2^{jB})=\left(\frac{c_1a_1^j+d_1^j}{r\log\left(\frac{\beta^j r_j}{c_1}\right)}, \frac{c_2a_2^j+d_2^j}{r_j\log\left(\frac{\beta^j r_j}{c_1}\right)} \right) 
	\end{equation}	
	else if $a_1^j+a_2^j= \frac{\beta^j r_j}{c_2}-1$
	\begin{equation}
		(\beta_1^{jB},\beta_2^{jB})=\left(\frac{\beta}{2}-\frac{c_2a_2^j-c_1a_1^j+d_2^j-d_1^j}{2r\log\left(\frac{\beta^j r_j}{c_2}\right)}, \frac{\beta^j}{2}+\frac{c_2a_2^j-c_1a_1^j+d_2^j-d_1^j}{2r_j\log\left(\frac{\beta^j r_j}{c_2}\right)} \right) 
	\end{equation}	
	or
	\begin{equation}
		(\beta_1^{jB},\beta_2^{jB})=\left(\frac{c_1a_1^j+d_1^j}{r_j\log\left(\frac{\beta^j r_j}{c_2}\right)}, \frac{c_2a_2^j+d_2^j}{r_j\log\left(\frac{\beta^j r_j}{c_2}\right)} \right) 
	\end{equation}	
	where $a_1$ and $a_2$ are given by Corollary 7.
\end{thm}}



==> Extra/regulatoryintervention.tex <==
\section{Regulatory intervention on ISP's effort}
In previous section, we observed that there is correlation between the effort by ISPs at equilibrium, and individual effort is not observable by CP. Therefore, as a regulatory intervention we propose that efforts have to be proportional to share proportion at equilibrium, i.e., $\frac{a_1}{a_2}= \frac{\beta_1^{E}}{\beta_2^{E}}$, where $\beta_i^{E}$ is the revenue share proportion corresponding to competitive scenario. Under this intervention, ISPs will put the effort in proportion to the share they get from CP. Now, we consider both cooperative and non-cooperative setup with this constraint.
\subsection{Competitive scenario}
Thus, the optimal effort by ISPs in response to the contract offered by the CP is given by
	$$ a_1+a_2= \frac{\beta_1 r}{c_1}-1$$
	and
	$$ a_1+a_2=\frac{\beta_2 r}{c_2}-1$$
	which implies 
	$$  \frac{\beta_1}{\beta_2}=\frac{c_1}{c_2}$$
	Given this, the optimal strategy for CP is to offer the contract that maximizes its utility, i.e., the solution to
	$$
	\max_{\beta_i\in [0,1], \sum_i\beta_i\le 1} (1-\beta_1-\beta_2)\log \left(\frac{\beta_1 r}{c_1}\right)
	$$
		\begin{thm} \label{beta}
		The equilibrium contract between CP and $ISP_i$ is given by
		$$\beta_i=\frac{c_i}{(c_1+c_2)W\left(\frac{r}{c_1+c_2}e\right)}; i=1,2 $$
	\end{thm}
	Using Theorem \ref{beta} and constraint $\frac{a_1}{a_2}=\frac{\beta_1}{\beta_2}$, one can characterize the equilibrium effort of ISPs.
	\begin{cor}
		There equilibrium effort by $ISP_i; i=1,2$ is given by:
		$$  a_i=\frac{c_i}{c_1+c_2}\left[\frac{r}{(c_1+c_2)W\left(\frac{r }{c_1+c_2}e\right)}-1\right]$$
	\end{cor}
	Now, having characterised equilibrium contract, we can now obtain utility of all the players.
\begin{cor}
    Utilities at equilibrium are given by
    \begin{enumerate}
        \item $U_{CP}=\frac{\left(W\left(\frac{re }{c_1+c_2}\right)-1\right)^2}{W\left(\frac{re }{c_1+c_2}\right)}$
        \item $U_{ISP_1}=\frac{c_1}{c_1+c_2}\left[r\left(1-\frac{2c_1+c_2}{(c_1+c_2)W\left(\frac{re }{c_1+c_2}\right)}\right)+c_1\right]$
             \item $U_{ISP_2}=\frac{c_2}{c_1+c_2}\left[r\left(1-\frac{2c_2+c_1}{(c_1+c_2)W\left(\frac{re }{c_1+c_2}\right)}\right)+c_2\right]$
    \end{enumerate}
\end{cor}	
\subsection{Cooperative scenario}
Under the cooperative setting, we first formulate Stage 1 problem, which is given by\\
CP:\\
$$\max_{\beta\in[0,1]} \quad (1-\beta)r\log(a_1+a_2+1)$$	
ISPs\\
$$\max_{a_1, a_2} \quad \beta r\log(a_1+a_2+1)-c_1a_1-c_2a_2$$
The best response by $ISP_2$ in response to the contract offered by CP is given by 
\begin{equation}
	a_1+a_2= \frac{\beta r}{c_1}-1 \quad \text{or} \quad 	a_1+a_2= \frac{\beta r}{c_2}-1 
\end{equation}
\begin{thm}
	The equilibrium contract between CP and ISPs given by 
	\begin{equation}
	\beta=\begin{cases} \frac{1}{W\left(\frac{r e }{ c_1}\right)} &\mbox{ if } 	a_1+a_2= \frac{\beta r}{c_1}-1, \\ \frac{1}{W\left(\frac{r e }{ c_2}\right)} &\mbox{ if } 	a_1+a_2= \frac{\beta r}{c_2}-1 \end{cases} 
	\end{equation}	
	\end{thm}
	Using constraint $\frac{a_1}{a_2}=\frac{\beta_1^{NE}}{\beta_2^{NE}}$, we obtain equilibrium efforts by ISP, given by following Corollary. 
\begin{cor}
	The effort by ISPs at equilibrium is given by
	\begin{equation}
		 a_i=\frac{c_i}{c_1+c_2}\left[\frac{r}{c_1W\left(\frac{r }{c_1}e\right)}-1\right]\text{or} \quad 		 a_i=\frac{c_i}{c_1+c_2}\left[\frac{r}{c_2 W\left(\frac{r }{c_2}e\right)}-1\right]
	\end{equation}
\end{cor}

\subsubsection{Nash Bargaining Solution}

Now, the Nash Bargaining problem for ISPs is given by:
\begin{align}\nonumber
	\max_{\beta_1} \quad \{\beta_1r\log(a_1+a_2+1)&-c_1a_1-d_1\}\times\\\nonumber
	\{(\beta-\beta_1)&r\log(a_1+a_2+1)-c_2a_2-d_2\}\\\nonumber
	\text{subjected to}\hspace{10mm}&\\ \nonumber
	\beta_1r\log(a_1+a_2+1)&-c_1a_1\ge d_1\\ \nonumber
	(\beta-\beta_1)r\log(a_1+a_2+1)&-c_2a_2\ge d_2
\end{align}
where $d_i=d_{ISP_i}, i=1,2$
\textcolor{}{\begin{thm} The NBS for the split of revenue share proportion between ISPs is given by \\
If $a_1+a_2= \frac{\beta r}{c_1}-1$
	\begin{equation}
		(\beta_1^B,\beta_2^B)=\left(\frac{\beta}{2}-\frac{c_2a_2-c_1a_1+d_2-d_1}{2r\log\left(\frac{\beta r}{c_1}\right)}, \frac{\beta}{2}+\frac{c_2a_2-c_1a_1+d_2-d_1}{2r\log\left(\frac{\beta r}{c_1}\right)} \right) 
	\end{equation}	
	or
	\begin{equation}
		(\beta_1^B,\beta_2^B)=\left(\frac{c_1a_1+d_1}{r\log\left(\frac{\beta r}{c_1}\right)}, \frac{c_2a_2+d_2}{r\log\left(\frac{\beta r}{c_1}\right)} \right) 
	\end{equation}	
	else if $a_1+a_2= \frac{\beta r}{c_2}-1$
	\begin{equation}
		(\beta_1^B,\beta_2^B)=\left(\frac{\beta}{2}-\frac{c_2a_2-c_1a_1+d_2-d_1}{2r\log\left(\frac{\beta r}{c_2}\right)}, \frac{\beta}{2}+\frac{c_2a_2-c_1a_1+d_2-d_1}{2r\log\left(\frac{\beta r}{c_2}\right)} \right) 
	\end{equation}	
	or
	\begin{equation}
		(\beta_1^B,\beta_2^B)=\left(\frac{c_1a_1+d_1}{r\log\left(\frac{\beta r}{c_2}\right)}, \frac{c_2a_2+d_2}{r\log\left(\frac{\beta r}{c_2}\right)} \right) 
	\end{equation}	
	where $a_1$ and $a_2$ are given by Corollary 7.
\end{thm}}	
\subsubsection{Shapley Value}
In this section, we study the Shapley value of ISPs when they are constrained by the regulatory intervention $\frac{a_1}{a_2}=\frac{\beta_1^{NE}}{\beta_2^{NE}}$. Following theorem gives Shapley values of ISPs.
\begin{thm} \label{SV}
Shapley value, $\Phi_i; i=1,2$ of ISPs is given as follows:\\
If $a_1+a_2=\frac{\beta r}{c_1}-1$
\begin{align}
      \Phi_1&=\frac{r}{2}\left(1-\frac{4}{W\left(\frac{re}{c_1}\right)}-\frac{2}{W\left(\frac{re}{c_2}\right)}\right)+c_1\\   \Phi_2&=\frac{r}{2}\left(1-\frac{2}{W\left(\frac{re}{c_2}\right)}\right)+c_2
\end{align}
 If $a_1+a_2=\frac{\beta r}{c_2}-1$   

\begin{align}
     \Phi_1&=\frac{r}{2}\left(1-\frac{2}{W\left(\frac{re}{c_1}\right)}\right)+c_1\\
      \Phi_2&=\frac{r}{2}\left(1-\frac{4}{W\left(\frac{re}{c_2}\right)}-\frac{2}{W\left(\frac{re}{c_1}\right)}\right)+c_2
\end{align}
\end{thm}

\subsection{Comparison between Cooperative and Non-Cooperative settings}
Now we will compare Cooperative and Non-Cooperative Solutions in terms of effort by ISPs and utilities of players. As the following result shows, the cooperative setting is always better for the CP, while numerical experiments show that non-cooperative setting can give higher payoff to $ISP_2$. The results are aligned with the case when only one ISP is putting a constant effort. 
\begin{thm} \label{thm:cmparision-2}
Under regulation intervention on efforts of ISPs, following statements holds
\begin{enumerate}
    \item  Total Effort is always higher when ISPs cooperate.
    \item  CP Utility is always higher when ISPs cooperate.
\end{enumerate}
\end{thm}
From Figs. 4-5, it can be seen that NBS is at least as good as non-cooperative equilibrium for ISPs. While on the other hand, Shapley value may be worst off for the ISP with less cost coefficient as compared to non-cooperative equilibrium. Therefore, NBS is always better for everyone including ISPs.


==> comparepublic.tex <==
In this section, we will now compare the cases when CP makes contract with public and private ISPs verses both private ISPs. In previous section, we show that cooperative scenario between private ISPs is always better for everyone as compared to competitive scenario. Our main result is the
following.
\begin{thm}
Suppose $r>c_i$. Following statements hold:
\begin{enumerate}
    \item Total profit shared by the CP is higher when all ISPs are private as compared to the case where one ISP is public.
    \item Total effort is higher in the presence of public ISP as compared to the case when all ISPs are private.
     \item CP Utility is higher in the presence of public ISP as compared to the case when all ISPs are private.
\end{enumerate}
\end{thm}
 



==> multipleISPs.tex <==
In this section, we study the case where CP makes profit sharing contract with multiple private ISPs ($n\geq 2$). We assume that $c_1\le c_2 \le \cdots \le c_n$. We first study the competitive scenario followed by the cooperative case. In competitive scenario, CP offers different revenue sharing contract with ISPs, each ISPs acts non-cooperatively to decide their respective effort. While in the cooperative scenario, we propose that CP offers a single joint contract to all the ISPs, where ISPs interact with each other and cooperatively  decide effort for the CP, and the revenue share split between them is in the ratio of their individual effort. 

\subsection{Competitive scenario}
In this section we consider the case where each ISP aims to selfishly maximize its utility.  Each ISP individually negotiates the contract with the CP while the CP aims to maximize the its profits from the efforts of all the ISPs. The objectives of the CP and the ISPs are given as:\\
CP (Leader):\\
$$\max_{\beta_i\in[0,1], \sum_i \beta_i\le1} \quad \left (1-\sum_i\beta_i\right)r\log \left (\sum_i a_i+1\right)$$
$ISP_i; i\in\mathcal{N}$ (follower: Private ISP)
$$\max_{a_i \ge 0} \quad \beta_ir\log \left (\sum_i a_i+1 \right)-c_ia_i$$
%Following proportion gives best response of each ISP to the contract offered by the CP.
% \begin{proposition} \label{effort-multiISP}
% Let $\{\beta_i\}$ denote the contract offered by the CP. Then the best response of the ISPs is such that 	
% \end{proposition}
% \textcolor{red}{It is strange to write this correlation here.
% Comparing the above set of equations, we get
% \begin{equation} \label{eqn:beta-ratio}
%     \frac{\beta_1}{c_1}=\frac{\beta_2}{c_2}=...=\frac{\beta_n}{c_n}
% \end{equation}
% }

% Given this, the optimal strategy for CP is to offer the contract that maximizes its utility, i.e., the solution to
% 	$$
% 	\max_{\beta_i\in [0,1], \sum_i\beta_i\le 1} (1-\sum_i\beta_i)\log \left(\frac{\beta_j r}{c_j}\right)
% 	$$
% 	The following result characterizes the equilibrium contracts between the CP
% 	and each ISP.
Solving the leader-follower game, we have the following equilibrium characterization. 
	\begin{thm} \label{thm:betaNC-multiISP}
	\textcolor{black}{Let $r>\sum_i c_i$}, at equilibrium 
	\begin{itemize}
	    \item the efforts of the ISPs is such that
	
	$$ \sum_{j \in \mathcal{N}} a_j^*= \frac{\beta_i r}{c_i}-1\quad \forall i\in \mathcal{N}$$
	\item the contracts offered by the CP is given by 
		$$\beta_i^*=\frac{c_i}{\sum_i c_iW\left(\frac{r}{\sum_j c_j}e\right)}\;\; \forall i\in \mathcal{N} $$
	\item the utility of the CP is 	
		  $$ U_{CP}=\frac{\left[W\left(\frac{r }{c_1+c_2}e\right)-1\right]^2}{W\left(\frac{r }{c_1+c_2}e\right)}r.$$
\end{itemize}		  
	\end{thm}
	Using Theorem \ref{thm:beta-NC}, one can characterize the equilibrium effort of ISPs.
% 	\begin{cor} \label{cor:effortNC-multiISP}
% 		There exist continuum of equilibria between ISPs given by:
	
% 	\end{cor}
	The above result implies that actions of ISPs are correlated with each other. The change in strategy of one ISP will impact the strategy of the other ISP. It is interesting to note that if one of the ISPs decreases it's effort, it will still get the same revenue share from the CP as the total effort is same. Such competitive scenario may lead to free riding by one of the ISPs, therefore, in the next section we propose cooperation between ISPs, whereby CP makes a joint payment to them and ISPs cooperatively decide the effort and the division of revenue share between them. 
	Because of continuum of equilibrium, it is not possible to compute utility of each ISP, but CP utility is still be computed as it depends on the total effort. 
% 	\begin{cor}
% 	    CP Utility at equilibrium is given by
	  
% 	\end{cor}
\begin{comment}	
\subsection{Cooperative scenario}	
We now study the cooperative setting, where ISPs jointly maximize their utilities to make the effort decision to improve the QoS for CP’s content. Further, CP pays a revenue share to ISPs jointly, and ISPs cooperatively decide the division between them. There are two stages under this case. 
\begin{itemize}
    \item \textit{Stage 1:} CP first announces a total share $\beta$ for both ISPs and ISPs  maximizes their sum utility to find the optimal effort for the CP. 
    \item \textit{Stage 2:} ISPs cooperatively decide the division of revenue share $\beta$, that depends on both effort, between them. We consider the outcome of division the share proportion $\beta$ by using the well-known cooperative solution concept of the \textit{Nash Bargaining solution}  (NBS). Nash Bargaining problem helps two players decide how to share a surplus generated by their joint actions. This solution concept satisfies important axioms which are: invariant to affine transformations, Pareto optimality, independence of irrelevant strategies and symmetry [8]. 
\end{itemize}

\subsubsection{Stage 1} Stage 1 problem constitutes joint payment of revenue share by CP to ISPs, and joint utility maximization by ISPs to make effort decision. The problem for Stage 1 is given as follows:\\
CP:
$$\max_{\beta\in[0,1]} \quad (1-\beta)r\log(a_1+a_2+1)$$	
ISPs:
$$\max_{a_1,a_2,...,a_n} \quad \beta r\log(\sum_i a_i+1)-\sum_i c_i a_i$$

\begin{proposition} \label{prop:effortstage1-multiISP}
	The optimal effort by ISPs is given either one of the following
	\begin{equation}
	\sum_i a_i= \frac{\beta r}{c_n}-1
	\end{equation}
\end{proposition}
Following Theorem characterize the equilibrium share proportion for ISPs, which depends upon the action by ISPs. 
\begin{thm} \label{thm:betastage1-multiISP}
For $r>c_i$, the equilibrium contract between CP and ISPs given by 
	\begin{equation}
\beta=\frac{1}{W\left(\frac{r e }{ c_n}\right)} 
	\end{equation}	
	\end{thm}


	\subsubsection{Stage 2}
Under this stage, ISPs can interact
and bargain with one another to arrive at a vector of revenue sharing contracts offered by CP, $(\beta_1^B,\beta_2^B,..., \beta_n^B)$, known as Nash Bargaining solution (NBS). Formally, the NBS is
defined as the solution of the following optimization problem:
$$\max_{\beta_i,\in[0,1]} \quad \prod_i\left(U_{ISP_i}(\beta_i)-d_{ISP_i}\right)$$
subjected to
$$U_{ISP_i}(\beta_i)\ge d_{ISP_i}$$
The disagreement point $d_{ISP_i}$ is taken to the utilities of $ISP_i$
corresponding to the case of competitive scenario in previous section.
Computation of NBS for $n>2$ is not analytically
tractable, therefore, we consider the of symmetric ISPs, where $c_i=c \forall i\in \mathcal{N}$. NBP for symmetric ISPs will give $\beta^B=\beta/n$. In the next section, we consider the case of two asymmetric ISPs.
\end{comment}
